Survey on 3D face reconstruction from uncalibrated images

Recently, a lot of attention has been focused on the incorporation of 3D data into face analysis and its applications. Despite providing a more accurate representation of the face, 3D facial images are more complex to acquire than 2D pictures. As a consequence, great effort has been invested in developing systems that reconstruct 3D faces from an uncalibrated 2D image. However, the 3D-from-2D face reconstruction problem is ill-posed, thus prior knowledge is needed to restrict the solutions space. In this work, we review 3D face reconstruction methods proposed in the last decade, focusing on those that only use 2D pictures captured under uncontrolled conditions. We present a classification of the proposed methods based on the technique used to add prior knowledge, considering three main strategies, namely, statistical model fitting, photometry, and deep learning, and reviewing each of them separately. In addition, given the relevance of statistical 3D facial models as prior knowledge, we explain the construction procedure and provide a list of the most popular publicly available 3D facial models. After the exhaustive study of 3D-from-2D face reconstruction approaches, we observe that the deep learning strategy is rapidly growing since the last few years, becoming the standard choice in replacement of the widespread statistical model fitting. Unlike the other two strategies, photometry-based methods have decreased in number due to the need for strong underlying assumptions that limit the quality of their reconstructions compared to statistical model fitting and deep learning methods. The review also identifies current challenges and suggests avenues for future research.

==> Sections/DeepLearning_old.tex <==
\section{Deep Learning Methods} \label{sec:DL}
% In the first two approaches for 3D-from-2D face reconstruction (statistical model fitting and photometric stereo), the prior knowledge needed to constrain the ill-posed problem is encoded in a 3D facial model or in a predefined template, or, as an alternative, a large collection of photos is used. In contrast, deep learning is able to learn the solutions space given a sufficiently large training set containing pairs of 2D images and their corresponding 3D faces.

The 3D-from-2D face reconstruction methods from the previous approaches (Sections \ref{sec:StatisticalModels} and \ref{sec:Photometry}) are based on modelling as a way of including prior knowledge: face model fitting methods include a geometry (and usually texture) model and photometric methods model the reflectance of the face. In contrast, deep learning methods directly learn the mapping between the 2D image and the 3D face, encoding prior knowledge in the weights of the trained network.

Although deep learning has shown to be a very powerful tool in many different applications, its potential in 3D-from-2D face reconstruction is limited due to the lack of ground truth 3D facial scans. To overcome this obstacle, researchers have proposed different approaches to construct training data sets together with different learning frameworks to alleviate the effect of the synthetic data in the training process.

In this section, we present and compare the most relevant works in 3D-from-2D face reconstruction that use deep learning as the main tool. Among the many elements that are involved in the learning process, we consider three representative ones, namely, 1) the training set used to train the network, 2) the learning framework and 3) the training criterion. We organise this section according to these items.

Table \ref{tab:DL} summarises the main characteristics of each of the reviewed deep learning works according to the above items. The \emph{training set} column indicates whether it was built by fitting a 3DMM to real images or by rendering synthetic images from a 3D face (or both). In the learning framework, four attributes are specified: the network type, the number of layers, if skip connections are used or not and if the learning process is iterative or not. The number of layers are indicated as $A\times B$ if the network is composed of $A$ networks of $B$ layers each and $X_1//X_2//\cdots//X_n$ if there are parallel networks with $X_1, \dots, X_n$ layers. Finally, the training criterion column indicates if the loss function is computed in a parameters space, the 3D space and/or the 2D space.





% \subsection{Network output}
% In 3D-from-2D face reconstruction, a deep neural network receives a facial image as input and generates the corresponding 3D face.

% Some works have directly estimated the 3D facial geometry represented as a 3D triangulated mesh \citep{BhagavatulaICCV2017,FLiuCVPR2018,SongTIP2012,LTranCVPR2018,TranCVPR2018}. Additionally, \citet{LTranCVPR2018} estimated the texture as a UV-map and the projection parameters. \citet{BhagavatulaICCV2017} also estimated the position of a set of landmarks in the input image since part of their contribution was face alignment. \citet{FLiuCVPR2018} trained the network to reconstruct the 3D face from the input image and to recognise the person, thus they also output the identity class of the person in the image.

% \begin{table*}[thp]
% \caption{Deep learning 3D-from-2D face reconstruction works that estimate 3DMM parameters. The parameters can be divided into shape (first column), texture (second column) and expression (third column). The fourth column indicates whether projection parameters are estimated.}
% \label{tab:3DMMparams_estimation}
% % \renewcommand{\arraystretch}{1.5}
% \renewcommand\tabularxcolumn[1]{m{#1}}
% \begin{tabularx}{\textwidth}{lYYYY}%cccc}
% \hline 
% & \textbf{Shape} & \textbf{Texture} & \textbf{Expression} & \textbf{Projection} \\ \hline
% \citet{JourablooCVPR2016,JourablooIJCV2017} & \cmark & & \cmark & \cmark \\ \hline
% \citet{Richardson3DV2016} & \cmark& \cmark & \cmark & \\ \hline
% \citet{XZhuCVPR2016} & \cmark& & \cmark & \cmark \\ \hline
% \citet{DouCVPR2017} & \cmark& & \cmark & \\ \hline
% \citet{RichardsonCVPR2017} & \cmark& \cmark & \cmark & \cmark \\ \hline
% \citet{TewariICCV2017,TewariCVPR2018} & \cmark& \cmark & \cmark & \cmark \\ \hline
% \citet{TranCVPR2017} & \cmark& \cmark & & \\ \hline
% \citet{KimCVPR2018} & \cmark& \cmark & \cmark & \cmark \\ \hline
% \citet{YGuoPAMI2018} & \cmark& \cmark & \cmark & \cmark \\ \hline
% \citet{GenovaCVPR2018} & \cmark& \cmark & & \\\hline
% \end{tabularx}
% \end{table*}

% Others, instead of estimating the 3D face directly, learnt the parameters of a 3DMM (see Table \ref{tab:3DMMparams_estimation}).

% In addition to the parameters specified in Table \ref{tab:3DMMparams_estimation}, \citet{TewariCVPR2018,TewariICCV2017} and \citet{KimCVPR2018} estimated the illumination of the input image using spherical harmonic functions under a Lambertian reflectance model.

% Apart from the 3DMM description of the face, other representations have been proposed. For example, \citep{GulerCVPR2017,YFengECCV2018,SelaICCV2017} used a depth representation (i.e. 2.5D) of the face. \citet{YFengECCV2018} used an UV-map to encode the 3D coordinates of the 3D reconstructed face. Similarly, \citet{SelaICCV2017} jointly estimated the UV-map and the correspondence between that UV-map and a 3D template face. Notice that if the UV-maps in the training set are in correspondence with a template mesh or a 3D facial model, the 3D facial mesh is easily recoverable. \citet{GulerCVPR2017} also estimated a UV-map, which, in this case, was in correspondence with a 3D facial template. They divided each dimension of the UV-space into $K$ bins and considered a representation of the $u$-coordinate (the same for the $v$-coordinate) that is divided into a discrete part $q$ and a residual part $r$, such that $u = q\cdot d + r$ (the same for $v$) where $d = 1/K$ is fixed.

% \citet{TrigeorgisCVPR2017} computed the surface normals and, in a post-processing step, the 3D facial shape was retrieved from the normals. \citet{JacksonICCV2017} proposed to represent the 3D faces as volumes by voxelisating them. The 3D facial shapes were then extracted as iso-surfaces of the estimated volumes.






\subsection{Training data set}
As we have mentioned above, the biggest obstacle when applying deep learning to 3D-from-2D face reconstruction is the lack of training data, since obtaining as many 3D facial scans as needed by deep learning algorithms is impractical. To overcome this limintation, researchers have proposed techniques for building synthetic training sets. These techniques take advantage of pre-built 3DMMs to obtain 3D faces in a much more accessible way.

We can distinguish two main approaches to build synthetic training sets. The first one is fitting a 3DMM to real images, and then rendering synthetic images using the estimated 3D faces. The second one is generating 3D faces by randomly sampling from a 3DMM and then, again, rendering synthetic images using the generated 3D faces. From now on, we will identify the first approach as \textit{Fit\&Render} and the second one as \textit{Generate\&Render}.

The \textit{Fit\&Render} approach was first introduced by \citet{XZhuCVPR2016}. They proposed a face profiling technique that is used to generate images across large poses, creating the 300W-LP (300W large poses) database. They first estimated a 3D mesh over the given face image by fitting a 3DMM using \citep{RomdhaniCVPR2005} and \citep{XZhuCVPR2015} over the background. Then, the 3D mesh was rotated and projected to the image to generate a synthetic image similar to the original one but with a large pose. This 300W-LP database has been used by many other authors \citep{BhagavatulaICCV2017,YFengECCV2018,GulerCVPR2017,JacksonICCV2017,LTranCVPR2018} since it includes realistic and challenging facial images with the ground truth 3DMM and projection parameters.

Similar to the \textit{Fit\&Render} strategy, some other works proposed to fit a 3DMM to images without rendering afterwards \citep{JourablooCVPR2016,JourablooIJCV2017,FLiuCVPR2018,TranCVPR2017,TranCVPR2018}. Whereas \citet{JourablooCVPR2016,JourablooIJCV2017} estimated the 3DMM parameters independently for each training image, \citet{FLiuCVPR2018} and \citet{TranCVPR2017,TranCVPR2018} combined parameters extracted from multiple images of the same person.

\citet{FLiuCVPR2018} fitted a 3DMM to multiple images enforcing common shape parameters to all the images of the same subject and estimating shape deformations for each image independently. In contrast, \citet{TranCVPR2017,TranCVPR2018} computed a weighted average of the shape and texture parameters estimated from the pictures of the same person. The resulting parameters were considered the ground-truth for all the images of that subject.

\citet{Richardson3DV2016} proposed a \textit{Generate\&Render} strategy based on a weak perspective projection and the Phong reflectance model to render the synthetic images. This approach was strictly followed by some \citep{DouCVPR2017,RichardsonCVPR2017,SelaICCV2017} and inspired others \citep{YGuoPAMI2018}. \citet{RichardsonCVPR2017} and \citet{SelaICCV2017} trained their networks using only the dataset generated by \citep{Richardson3DV2016}, unlike \citet{DouCVPR2017}, who also used publicly available 3D face databases, namely, the FRGC2 database \citep{PhillipsPAMI2009_FRGC2_DB}, the BU-3DFE database \citep{YinFG2006_BU-3DFE_DB} and the UHDB31 database \citep{WuISBA2016_UHDB31_DB}.

\citet{YGuoPAMI2018} also followed the strategy presented by \citep{Richardson3DV2016}. However, they considered that the rendered images in \citep{Richardson3DV2016} were not sufficiently photo-realistic. To address this shortcoming, they proposed an inverse rendering method, which they used to create their own synthetic training set.

Following the same strategy of \textit{Generate\&Render}, \citep{SenguptaCVPR2018,GenovaCVPR2018} trained their networks in a two stage manner. \citet{SenguptaCVPR2018}, in the first stage, trained a simple network over synthetic data extracted using the \textit{Generate\&Render} technique. In the second stage, they used the pre-trained simple network to label real images. The training data set for the 3D-from-2D face reconstruction network was composed of synthetic 3D-2D data and 2D real images with the estimated labels, which they claimed prevented the network to produce trivial solutions. In contrast, \citet{GenovaCVPR2018} proposed to train their face reconstruction network with unlabelled, although, in a previous stage, they pre-trained it with synthetic 3D-2D data (generated following the \textit{Generate\&Render} strategy).

%in the first stage, pre-trained their face reconstruction network with synthetic 3D-2D data (generated following the \textit{Generate\&Render} strategy). In the second stage, they used unlabelled real images.



The two main strategies, \textit{Fit\&Render} and \textit{Generate\&Render}, were combined by \citep{TrigeorgisCVPR2017,KimCVPR2018}. \citet{TrigeorgisCVPR2017} constructed their training dataset using different databases. They used the ICT-3DRFE database \citep{StratouFG2011_3DRFE_DB} and the Photoface database \citep{ZafeiriouCVPR2011_PhotofaceDB} to generate synthetic images varying the illumination. They followed the \textit{Fit\&Render} strategy using the LSFM \citep{BoothIJCV2017_LSFM} as 3DMM and adding expressions with the FaceWarehouse model \citep{CaoVCG2014_FaceWarehouseFM}. With the same facial model, they also followed the \textit{Generate\&Render} strategy. These randomly generated 3D faces were aligned to in-the-wild images to provide realistic backgrounds to the rendering. \citet{KimCVPR2018} built a first training set using \textit{Generate\&Render} to pre-train the network. Then, during iterative training, they followed the \textit{Fit\&Render} strategy using the pre-trained network to estimate the model parameters from real images. Gaussian noise was added to these estimated parameters before rendering synthetic images, which were used to train the network in the next iteration.

Although most of the works built training sets generated following one of the two main strategies, there are others that followed none of them. \citet{SongTIP2012} trained their network using only real data: real 2D images and real 3D scans from the BU-3DFE database \citep{YinFG2006_BU-3DFE_DB}. \citet{TewariCVPR2018,TewariICCV2017} and \citet{LTranCVPR2018} trained their networks in an unsupervised manner, which enables to train the networks end-to-end without the need of ground truth 3D faces.





\subsection{Learning framework}
The core part of a deep leaning algorithm is the network itself, in terms of its architecture and how it learns its weights. The most straightforward learning framework is a single neural network that is trained in a feed-forward manner (Section \ref{subsubsec:FeedForward}), in contrast to encoder-decoder networks (Section \ref{subsubsec:EncDec}) and cascaded regressors (Section \ref{subsubsec:Cascaded}), which are constructed by stacking several networks together. Other approaches used various networks but each one of them was trained for an specific task. In multi-stage approaches (Section \ref{subsubsec:MultiStage}) these tasks are independent, whereas in coarse-to-fine approaches (Section \ref{subsubsec:Coarse2Fine}) one network refines the output of the other. Other researchers added sub-networks, which are also trained for specific tasks, to a main network (Section \ref{subsubsec:SubNets}). Finally, an iterative learning framework have been explored where the output of the network is iteratively refined (Section \ref{subsubsec:Iterative}).




\subsubsection{Feed-forward - whatever} \label{subsubsec:FeedForward}
\citet{TrigeorgisCVPR2017} and \citet{TranCVPR2017} used a residual convolutional neural network, the ResNet architecture \citep{HeCVPR2016_ResNet}. The first authors \citep{TrigeorgisCVPR2017} trained the ResNet-50 (50 layers) network to estimate the facial normals from a single image. \citet{TranCVPR2017} used the ResNet-101 network (101 layers) to estimate the parameters of 3DMM. Instead, \citet{TewariCVPR2018} used a feed forward convolutional neural network (CNN) based on the AlexNet architecture \citep{KrizhevskyNIPS2012_AlexNet}. This network estimated a 3DMM parameters (shape, geometry and expression), which generate a coarse 3D face from which they estimate medium-level corrections as per-vertex displacements.


\subsubsection{Encoder-Decoder} \label{subsubsec:EncDec}
The encoder-decoder architecture allows to train a network to extract features from the input facial image (encoder) which are then decoded (decoder). The methods that used this encoder-decoder architecture can be divided into two groups: the ones whose encoder already estimates the 3D face and the decoder generates a synthetic 2D image matching the input one, and the ones whose decoder recovers a representation of the 3D face from the enconder's output.

\citet{TewariICCV2017} and \citet{LTranCVPR2018} correspond to the first group. \citet{TewariICCV2017} used a predefined architecture as encoder and added a simple architecture as decoder. Their encoder, the AlexNet network \citep{KrizhevskyNIPS2012_AlexNet}, estimated all the 3DMM parameters together with the rendering parameters. These parameters were the input for the decoder, which consisted of a single layer that rendered a synthetic image from the 3D face estimated by the encoder. Instead, \citet{LTranCVPR2018} proposed to use two CNN decoders: one converted the shape features estimated by the encoder (a CNN) into a 3D shape, and the other decoder transforms the texture features into an UV texture map. The learning framework employed by \citet{TewariICCV2017} and \citet{LTranCVPR2018}, allows them to train their networks in an unsupervised manner.


The following methods belong to the second group of encoder-decoder approaches, where the decoder reconstructs the 3D face from features extracted by the encoder.

\citet{SongTIP2012} formed the encoder-decoder architecture by stacking together two radial basis function networks. Each one of the networks learned an intrinsic representation of the 3D faces (\textit{3D-network}) and the 2D cropped facial images (\textit{2D-network}), respectively. For a pair of 2D-3D data of the same person, the intrinsic representation had to be very similar for both the 2D image and the 3D face. Thus, the encoder-decoder network was constructed by stacking the \textit{2D-network} (encoder) and the inverted \textit{3D-network} (decoder): the network inputs a 2D facial image and the encoder estimates its intrinsic representation, which in turn is the input for the inverted 3D-network (decoder) that outputs the 3D face.

\citet{SelaICCV2017} and \citet{YFengECCV2018} used the encoder-decoder learning framework to estimate depth maps from the input images. The first one \citep{SelaICCV2017} based their network on the U-Net architecture \citep{RonnebergerMICCAI2015_UNet}, where skip connections are used between corresponding layers in the encoder and the decoder. The network's output is a depth map and a correspondence map from each pixel of the image to a vertex on a reference mesh, with which they built a coarse facial mesh. From this coarse mesh and the input image, fine details are reconstructed by estimating a displacement map. \citet{YFengECCV2018} proposed a residual CNN with an encoder-decoder architecture where the encoder mapped the input image to a feature map and the decoder converted this feature map into a position map which contains the XYZ coordinates of the ground truth shape .

\citet{GenovaCVPR2018} and \citet{FLiuCVPR2018} proposed decoders with simple architectures. The first one \citep{GenovaCVPR2018} used the FaceNet network \citep{SchroffCVPR2015_FaceNet} as the encoder and a network with two fully-connected layers served as decoder to estimate the 3DMM parameters. \citet{FLiuCVPR2018} used the SphereFace network \citep{LiuCVPR2017_SphereFace} to estimate separately identity and identity-irrelevant features. Two different multilayer perception networks were used as decoders, which output the identity and identity-irrelevant difference with respect to a mean shape. The final reconstruction was computed adding these differences to the mean shape.


Differently from all the previous works, \citet{JacksonICCV2017} proposed to stack two encoder-decoder networks. Each network is an hourglass network \citep{NewellECCV2016_HourglassNet}, which uses skip connections and residual modules. According to \citet{JacksonICCV2017}, stacking two encoder-decoder networks allows to refine the output of the first network with the second one.




\subsubsection{Cascaded Regressor} \label{subsubsec:Cascaded}
Another learning framework that has been used is the cascaded regressor, where each regressor is a convolutional neural network. Each CNN estimates an update of the input parameters, which are estimated by the previous regressor, such that it is closer to the ground truth.

\citet{XZhuCVPR2016} proposed to estimate the update of all the parameters of the model (3DMM and projection parameters) at the same time. In contrast, \citet{JourablooCVPR2016,JourablooIJCV2017} considered two different regressors that were alternated, one that estimated the 3DMM parameters updates and the other that estimated the projection parameters updates. Whereas in \citep{JourablooCVPR2016}, they used a ``simple'' CNN, in \citep{JourablooIJCV2017}, they changed all the regressors but the first. The new CNN they used followed a Siamese network \citep{BromleyNIPS1993_SiameseNet} that has two branches with shared weights. The input of this network is the original face image together with its mirrored image. This allows ensuring that the estimated update of the 2D landmarks (projection of the 3D landmarks) for both the input image and the mirrored image are similar.



\subsubsection{Multi-stage} \label{subsubsec:MultiStage}
\citet{SenguptaCVPR2018} and \citet{BhagavatulaICCV2017} considered a multi-stage learning framework, where different specific tasks are carried out in each stage.

\citet{SenguptaCVPR2018} used a network containing residual and convolutional blocks. The architecture of the network was designed to learn to separate low and high frequency variations into normals and albedo. Then, the normals, the albedo and the input image were jointly used to learn the lighting parameters. \citet{BhagavatulaICCV2017} estimated the 3D face by deforming a template according to some learnt warping parameters. They extracted features form the image using a pretrained network. These features were the input of two different networks that extracted the warping and the projection parameters respectively. Then, the 3D face was built using the estimated parameters, and the 3D landmarks were projected into the image. Finally, the projected 3D landmarks were refined by extracting features from each of them and estimating their offset with a fully connected layer.




\subsubsection{Coarse-to-Fine} \label{subsubsec:Coarse2Fine}
% which separate global shape from local details. This separation allows for strong regularization over the global face shape – thereby providing robustness even in the most challenging viewing conditions – and weak regularization over the local details.


Similar to the multi-stage learning framework, \citet{RichardsonCVPR2017} and \citet{YGuoPAMI2018} used a coarse-to-fine framework, where each stage estimates finer details than the previous one. \citet{RichardsonCVPR2017} proposed to use two different networks, one that estimated the coarse 3D face (CoarseNet) and the other that refined it (FineNet). The CoarseNet's architecture was based on the ResNet network \citep{HeCVPR2016_ResNet}, and iteratively estimated the 3DMM and projection parameters by adding a feedback channel. The resulting parameters were then converted into a depth map, which was the input of the FineNet based on the hypercolumn architecture \citep{HariharanCVPR2015_HypercolumnNet} with the VGG-Face network \citep{ParkhiBMVC2015_VGGFace} as a base. This work \citep{RichardsonCVPR2017} inspired \citet{YGuoPAMI2018} to apply the coarse-to-fine framework to videos instead to single images. To do so, they included a Tracking CoarseNet that predicted the next frame's coarse parameters.

In their later work, \citet{TranCVPR2018} used their previous work \citep{TranCVPR2017} to estimate a coarse 3D face that is later refined. The fine details are represented by a bump map which is estimated from the image as per-vertex depth displacements. To estimate these bump maps, they trained the encoder-decoder network from \citep{IsolaCVPR2017_Img2Img} with ground truth bump maps generated by \citep{OrElCVPR2015}.


\subsubsection{Sub-networks} \label{subsubsec:SubNets}

\citet{DouCVPR2017} and \citet{GulerCVPR2017} proposed architectures where sub-networks with specific tasks were attached to a main common network. The network proposed in \citep{DouCVPR2017} has a sub-CNN that combined features from intermediate layers of the common VGG-Face network \citep{ParkhiBMVC2015_VGGFace}. This sub-CNN estimated expression-specific features while the main network, VGG-Face, estimated the identity-specific features. Both type of features were then combined to form a 3D face. \citet{GulerCVPR2017} proposed to add branches at the end of a ResNet-based network \citep{HeCVPR2016_ResNet} to estimate separately the U-coordinates and the V-coordinates of an UV-map.


\subsubsection{Iterative} \label{subsubsec:Iterative}
A very different learning framework was adopted by \citet{Richardson3DV2016} and \citet{KimCVPR2018}. Both reconstruct the 3D face from a 2D facial image by iteratively refining the output of the network. In \citep{Richardson3DV2016}, Richardson et al. proposed to add a secondary input channel that inputs a rendered image using the previous output parameters. Thus, iteratively, the network, which was based on the ResNet network \citep{HeCVPR2016_ResNet}, was trained to correct the previous prediction. \citet{KimCVPR2018} incremented the training set in each iteration by adding synthetic images that were rendered using parameters (after adding a Gaussian noise) estimated with the currently-trained network from real images. Thus, in the next iteration, the network was trained over a training set the ``previous'' network generated. In this way, the training data distribution was more similar to the real distribution, alleviating the effect of the synthetic data in the training process.






\subsection{Training criterion}
To train a deep leaning network, another decisive element is the training criterion, i.e the loss function (also called the cost or the error function) minimised by the network in the training process. Evidently, this loss function depends directly on the output of the network since, roughly, it minimises the error between the estimated output and the ground truth.

% PARAMS ERROR
% Leave Jourabloo at the end so it links with LMKS ERROR with Bhagavatula (3D FACES ERROR)
Most of the works presented above estimated the parameters of a 3DMM from the input image. Among them, a popular term included in the cost function is the error between the estimated and the ground truth parameters \citep{GenovaCVPR2018,JourablooCVPR2016,JourablooIJCV2017,KimCVPR2018,SenguptaCVPR2018,TranCVPR2017,TranCVPR2018,XZhuCVPR2016}.

\citet{TranCVPR2017,TranCVPR2018} used the \textit{asymmetric Euclidean loss}, which decouples the under-estimation and over-estimation errors
\begin{align*}
 \mathbb{E}_{\text{asym}}(\vec{\theta},\vec{\theta}_\text{gt}) & = w_1 \norm{\text{abs}(\vec{\theta}_\text{gt}) - \max(\vec{\theta},\vec{\theta}_\text{gt})} + \\
 & \quad \ w_2 \norm{\text{abs}(\vec{\theta}) - \max(\vec{\theta},\vec{\theta}_\text{gt})}.
\end{align*}
In addition, in \citep{TranCVPR2018} they included a loss function to learn to predict the bump map $\vec{\Delta}$ that refines the 3D face estimated by \citep{TranCVPR2017}. This \textit{bump loss} computes the error of the estimated bump map, including the difference between the gradient of the estimated and the ground truth bump maps to favour smoother surfaces
\begin{align*}
 \mathbb{E}_{\text{bump}}(\vec{\Delta},\vec{\Delta}_\text{gt}) &= \norm{\vec{\Delta} - \vec{\Delta}_\text{gt}}_1 + \norm{\frac{\partial \vec{\Delta}}{\partial x} - \frac{\partial \vec{\Delta}_\text{gt}}{\partial x}}_1 + \\ 
 & \quad \norm{\frac{\partial \vec{\Delta}}{\partial y} - \frac{\partial \vec{\Delta}_\text{gt}}{\partial y}}_1.
\end{align*}


\citet{KimCVPR2018}, \citet{XZhuCVPR2016} and \citet{GenovaCVPR2018} used a \textit{weighted parameters distance cost}, which computes the Euclidean distance between the vector of estimated parameters $\vec{\theta}$ and the vector of ground truth parameters $\vec{\theta}_{\text{gt}}$ but with weighting factors for each parameter to balance their global importance
\begin{equation*}
 \mathbb{E}_{\text{wpdc}}(\vec{\theta},\vec{\theta}_\text{gt}) = (\vec{\theta} - \vec{\theta}_\text{gt})^\text{T} \vec{W} (\vec{\theta} - \vec{\theta}_\text{gt}).
\end{equation*}
The main difference between each of them is the weighting matrix. \citet{KimCVPR2018} proposed to use a weight matrix $\vec{W} = \vec{\Sigma}^\text{T} \vec{\Sigma}$ where $\vec{\Sigma}$ is a diagonal matrix with weights that incorporate the standard deviation of each parameter, $\sigma_i$, $\vec{\Sigma} = \text{diag}(\sigma_1 w_1,\dots, \sigma_K w_K)$. The weight matrix used by \citet{XZhuCVPR2016} was a diagonal matrix $\vec{W} = \text{diag}(w_1,\dots,w_K)$ where
\begin{equation*}
 w_i = \frac{\norm{\mathcal{P}(\vec{x}(\tilde{\vec{\theta}}^{[i]}),\tilde{\vec{\theta}}^{[i]}) - \mathcal{P}(\vec{x}(\vec{\theta}_\text{gt}),\vec{\theta}_\text{gt})}_2}{\sum_{k=1}^K w_k}.
\end{equation*}
$\tilde{\vec{\theta}}^{[i]}$ is defined as the vector of parameters where the $i$th element comes from the estimated parameter $\tilde{\theta}^{[i]}_i = \theta_i$ while the rest come from the ground truth $\tilde{\theta}^{[i]}_j = \theta_{j,\text{gt}}$, $\forall j\neq i$. $\vec{x}(\vec{\theta})$ defines the 3D facial shape built with the shape and expression parameters from $\vec{\theta}$, and $\mathcal{P}(\vec{x}(\vec{\theta}),\vec{\theta})$ defines the projection of $\vec{x}(\vec{\theta})$ according to the projection parameters in $\vec{\theta}$. \citet{GenovaCVPR2018} used a common weight for all the parameters of the same space, i.e., one weight for the shape parameters and another for the texture parameters. Additionally, they used another two terms: identity loss and batch distribution loss. The first ensures that the encoder extracts similar features $\vec{f}$ from images of the same person by computing the cosine similarity $\mathbb{E}_{\text{id}}(\vec{f}_i,\vec{f}_j) = \vec{f}_i \cdot \vec{f}_j$. This term is used to compute the similarity of the ID-features extracted from a real image and the image rendered using the parameters estimated by the decoder over the real input image.

\citet{JourablooCVPR2016,JourablooIJCV2017} and \citet{SenguptaCVPR2018} used a loss function over the parameters that consisted simply on computing the $q$-norm of the difference between the estimated and the ground truth parameters
\begin{equation} \label{eq:error_qnorm}
 \mathbb{E}_{\text{q-norm}}(\vec{\theta},\vec{\theta}_\text{gt}) = \norm{\vec{\theta} - \vec{\theta}_\text{gt}}_q = \sum_{i=1}^K | \theta_i - \theta_{i,\text{gt}} |^q.
\end{equation}

\citet{SenguptaCVPR2018} used a loss function composed of four terms $\mathbb{E} = w_{\vec{n}} \mathbb{E}_{\vec{n}} + w_{\vec{\beta}}\mathbb{E}_{\vec{\beta}} + w_{\vec{\gamma}} \mathbb{E}_{\vec{\gamma}} + w_{\vec{I}}\errorI$. On the one hand, the error over the surface normals, $\mathbb{E}_{\vec{n}}(\vec{n},\vec{n}_\text{gt})$, the error over the texture 3DMM parameters, $\mathbb{E}_{\vec{\beta}}(\vec{\beta},\vec{\beta}_\text{gt})$ and the error over the images, $\errorI(\Imod,\Iin)$ (where $\Iin$ is the input real image and $\Imod$ is the rendered image using the current parameters) were computed with the $L_1$ norm ($q = 1$ in eq. \eqref{eq:error_qnorm}). On the other hand, the error over the lighting parameters, $\mathbb{E}_{\vec{\gamma}}(\vec{\gamma},\vec{\gamma}_\text{gt})$, was computed using the $L_2$ norm ($q=2$ in eq. \eqref{eq:error_qnorm}).

\citet{JourablooCVPR2016,JourablooIJCV2017} used the $L_2$ norm error to estimate the parameters update in the cascaded CNN they proposed. Thus, in eq. \eqref{eq:error_qnorm}, $\vec{\theta}_\text{gt}$ is the ground truth update (difference between current estimate and ground truth parameters) and $\vec{\theta}$ is the update estimated by the current CNN. In addition, in \citep{JourablooIJCV2017} they also estimated the location of the 2D landmarks in the input face, thus they include a landmark term that ensures the landmarks on the input face are similar to the landmarks on the mirrored image (with a reordering). This term minimises the $L_2$ norm of the difference between the projected landmarks over the original image and over the mirrored image.

% 3D FACES ERROR
Unlike the works above that proposed loss functions that minimise the parameters error, others computed the Euclidean loss ($q=2$ in eq. \eqref{eq:error_qnorm}) over the 3D faces directly, \citep{BhagavatulaICCV2017,DouCVPR2017,FLiuCVPR2018,Richardson3DV2016,RichardsonCVPR2017}. \citet{BhagavatulaICCV2017} and \citet{FLiuCVPR2018} output the regressed 3D, whereas \citet{DouCVPR2017} and \citet{Richardson3DV2016,RichardsonCVPR2017} output 3DMM parameters. Thus, to apply the Euclidean loss to the 3D faces, first the 3D geometry (and texture in some cases) have to be recovered by multiplying the model basis to the estimated parameters.

To also train the network on face recognition, \citet{FLiuCVPR2018} added to the Euclidean loss a softmax loss that served as a face identification error. \citet{BhagavatulaICCV2017} added an Euclidean loss over the 2D regressed landmarks so the network also learned to estimate the 2D landmarks over the input image. Finally, to refine the depth map estimated by the coarse network, $\vec{z}_{\text{c}}$ (trained only using the Euclidean loss), \citet{RichardsonCVPR2017} applied a loss function that consisted of three terms. One was an image term that computes the Euclidean distance between the original image and the rendered image according to the current parameters and depth map. Another was a fidelity term to ensure the estimated map does not differ much from the coarse depth map, $\mathbb{E}_\text{fidel} (\vec{z})= \norm{\vec{z} - \vec{z}_{\text{c}}}_2^2$. And the last was a smoothness term to ensure the gradient of the map is not large, $\mathbb{E}_{\text{smooth}} = \norm{\vec{\Delta}z}_1$, where $\vec{\Delta}$ is the Laplacian operator.

% IMAGE ERROR (unsupervised?)
% Introduced with Richardson, continue with YGuo and Sengupta.
% Leave Tewari and LTran at the end since they are unsupervised.
Like \citet{SenguptaCVPR2018} and \citet{RichardsonCVPR2017}, others have used the image error computed as the Euclidean distance between the input image and the image rendered with the estimated parameters \citep{TewariICCV2017,TewariCVPR2018,LTranCVPR2018}. Unlike \citet{SenguptaCVPR2018}, \citep{RichardsonCVPR2017,TewariICCV2017,TewariCVPR2018,LTranCVPR2018} used the image error to drive the learning in an unsupervised manner, which in \citep{TewariICCV2017,TewariCVPR2018,LTranCVPR2018} was also driven using a 2D landmarks error. Whereas \citet{TewariICCV2017,TewariCVPR2018} complemented the image and landmark errors with regularisation terms, \citet{LTranCVPR2018} added an adversarial loss, training a discriminator network to distinguish between real images and images rendered by the generator (the network proposed to reconstruct 3D faces from 2D images) while training the generator to produce more realistic faces.

Other loss functions have been used. \citet{YGuoPAMI2018} trained their coarse network by computing the Euclidean distance between the projection of the 3D faces built from the ground truth and estimated parameters. However, to be able to control the effect the projection parameters and the geometry parameters individually, the estimated 3D face was projected considering the projection parameters as the estimated values and the geometry parameters as the ground truth values (and the other way around)
\begin{align*}
 &\mathbb{E} = w \mathbb{E}_\text{proj} + (1-w)\mathbb{E}_\text{geo}\\
 &\text{where}\\
 &\mathbb{E}_\text{proj} = \norm{\mathcal{P}(\vec{x}(\vec{\theta}_\text{geo}^\text{gt}),\vec{\theta}_\text{proj}) - \mathcal{P}(\vec{x}(\vec{\theta}_\text{geo}^\text{gt}),\vec{\theta}_\text{proj}^\text{gt})}^2_2 \text{ and}\\
 &\mathbb{E}_\text{geo} = \norm{\mathcal{P}(\vec{x}(\vec{\theta}_\text{geo}),\vec{\theta}_\text{proj}^\text{gt}) - \mathcal{P}(\vec{x}(\vec{\theta}_\text{geo}^\text{gt}),\vec{\theta}_\text{proj}^\text{gt})}^2_2.
\end{align*}
$\mathcal{P}(\vec{x}(\vec{\theta}_\text{geo}),\vec{\theta}_\text{proj})$ indicates the projection of the 3D face built from the geometry parameters $\vec{\theta}_\text{geo}$, $x(\vec{\theta}_\text{geo})$, according to the projection parameters $\vec{\theta}_\text{proj}$. In the tracking network, to this loss function, they added an image error term and they trained the fine network with an Euclidean distance loss between the ground truth and the estimated displacement map.

\citet{SongTIP2012} trained the coupled radial basis function network with a loss function that consists of a reconstruction error, a smoothness regularisation term and a point distribution consistency. The first ensures that both networks (and their inverted networks) can be stacked together by minimising the difference between the input of one and the output of the other. The second minimises the energy of the gradient of the map that converts a 2D image (or 3D face) into an intrinsic representation and the gradient of its inverse. And the third makes the distributions of two sets of intrinsic representations (one from 3D and the other from 2D) similar to each other.

\citet{JacksonICCV2017} used the sigmoid cross-entropy loss to train the proposed hourglass network to estimate the volumetric representation of a face. \citet{TrigeorgisCVPR2017} compared two different losses to learn to estimate surface normals from facial images: the angular distance between the estimated and the ground truth normals, $\mathbb{E} = 1 - \sum_i \vec{n}_i^\text{T}\vec{n}_{i\text{,gt}}$, and the smoothed version of the $L_1$ norm proposed by \citep{GirshickICCV2015_smoothL1}.

\citet{GulerCVPR2017}, \citet{SelaICCV2017} and \citet{YFengECCV2018} proposed three different ways to train a network to estimate a depth representation of the 3D face. The first \citep{GulerCVPR2017} divided each dimension of the UV-space into a discrete part and a residual part. They used the softmax cross-entropy loss to estimate the discrete part and the smoothed version of the $L_1$ norm proposed by \citep{GirshickICCV2015_smoothL1} to estimate the residual part. \citet{SelaICCV2017} proposed a loss function that is a linear combination of the $L_1$ norm over the difference between the estimated and ground truth depth maps and the $L_1$ norm of the difference between the normals of both depth maps. Finally, \citet{YFengECCV2018} proposed a loss function that computes the Euclidean distance between the ground truth and the estimated position UV-maps with a weight mask that assigns a weight to each pixel in the map to penalise errors on the facial regions that have more discriminative features.



\begin{table*}[thp]
\caption{3D-from-2D face reconstruction approaches based on deep learning.} \label{tab:DL}
% \renewcommand{\arraystretch}{1.3}
\renewcommand\tabularxcolumn[1]{m{#1}}
\begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}m{0.4cm}Y|m{1.6cm}m{2.2cm}XX|YYY}%{XllXXXX}%{Xlm{1.2cm}m{2.45cm}m{2.65cm}m{2.58cm}X}
\hline
\multirow{2}{*}{Reference} & \multicolumn{2}{l|}{Training set} & \multicolumn{4}{l|}{Learning framework} & \multicolumn{3}{l}{Training criterion}\\ \cline{2-10}
& Fit & Render & Network type & \# Layers & Skip connect. & I\-te\-ra\-ti\-ve & Param. space & 3D space &2D space\\ \hline

\multirow{2}{*}{\cite{SongTIP2012}} & \multicolumn{2}{c|}{\multirow{2}{*}{Real data}} & Encoder & 3 & No & No & \multirow{2}{*}{x} & \multirow{2}{*}{} & \multirow{2}{*}{} \\
 & \multicolumn{2}{l|}{} & Decoder & 3 & No & No & & & \\ \hline

\cite{XZhuCVPR2016} & x & x & CNN & 6 & No & Yes & x  & &  \\ \hline

\cite{Richardson3DV2016} & & x & Residual & 18 & Yes & Yes & & x  &  \\ \hline

\cite{JourablooCVPR2016} & x & & CNN & 6 & No & Yes & x  & &  \\ \hline
\multirow{2}{*}{\cite{JourablooIJCV2017}} & \multirow{2}{*}{x} & \multirow{2}{*}{} & CNN & 5 & No & No & \multirow{2}{*}{x} & \multirow{2}{*}{} & \\
 & & & CNN & 6 & No & Yes & & & x   \\ \hline

\multirow{2}{*}{\cite{BhagavatulaICCV2017}} & \multirow{2}{*}{x} & \multirow{2}{*}{x} & CNN & 8 (16)\setfootnotemark\label{first} & No & No & \multirow{2}{*}{} & \multirow{2}{*}{x} & \multirow{2}{*}{} \\
 & & & FC & \#lmks//4//4 & No & No & & & \\ \hline

\multirow{2}{*}{\cite{DouCVPR2017}} & \multirow{2}{*}{} & \multirow{2}{*}{x} & CNN & 16 & No & No & \multirow{2}{*}{} & \multirow{2}{*}{x} & \multirow{2}{*}{}  \\
 & & & CNN & 19 & Yes & No & & & \\ \hline

\multirow{2}{*}{\cite{GulerCVPR2017}} & \multirow{2}{*}{x} & \multirow{2}{*}{x} & Residual & 101 & Yes & No & \multirow{2}{*}{x}  & \multirow{2}{*}{} & \multirow{2}{*}{}\\
& & & FC & $4\times 1$ & No & No & & &  \\ \hline

\multirow{2}{*}{\cite{JacksonICCV2017}} & \multirow{2}{*}{x} & \multirow{2}{*}{x} & Encoder & 6 & Yes & No & \multirow{2}{*}{} & \multirow{2}{*}{x} & \multirow{2}{*}{} \\
 & & & Decoder & 5 & Yes & No & & & \\ \hline

\multirow{2}{*}{\cite{RichardsonCVPR2017}} & \multirow{2}{*}{} & \multirow{2}{*}{x} & Residual & 19 & Yes & Yes & \multirow{2}{*}{} & \multirow{2}{*}{x} & \multirow{2}{*}{x}  \\
 & & & CNN & 16 & No & No & & &  \\ \hline

\multirow{2}{*}{\cite{SelaICCV2017}} & \multirow{2}{*}{} & \multirow{2}{*}{x} & Encoder & 8 & Yes & No & \multirow{2}{*}{} & \multirow{2}{*}{x} & \multirow{2}{*}{} \\
 & & & Decoder & 8 & Yes & No & & &  \\ \hline

\cite{TewariICCV2017}& x & & CNN & 8 & No & No & & & x   \\ \hline

\cite{TrigeorgisCVPR2017}& x & x & Residual & 50 & Yes & No & & x  &  \\ \hline

\cite{TranCVPR2017} & x & & Residual & 101 & Yes & No & x  & &  \\ \hline

\multirow{3}{*}{\cite{TranCVPR2018}} & \multirow{3}{*}{x} & \multirow{3}{*}{} & Residual & 101 & Yes & No & \multirow{3}{*}{x} & \multirow{3}{*}{} & \multirow{3}{*}{} \\
 & & & Encoder & 8 & Yes & No & & & \\
 & & & Decoder & 8 & Yes & No & & &  \\ \hline

\multirow{2}{*}{\cite{FLiuCVPR2018}} & \multirow{2}{*}{x} & \multirow{2}{*}{} & Encoder & 21 & No & No & \multirow{2}{*}{} & \multirow{2}{*}{x} & \multirow{2}{*}{} \\
 & & & Decoder & $2\times1$ & No & No & & &  \\ \hline

\cite{KimCVPR2018} & x & x & CNN & 8 & No & Yes & x  & &  \\ \hline

\multirow{2}{*}{\cite{LTranCVPR2018}} & \multirow{2}{*}{x} & \multirow{2}{*}{x} & Encoder & 14 & No & No & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{x} \\
 & & & Decoder & 15 // 17 & No & No & & &  \\ \hline

\multirow{3}{*}{\cite{SenguptaCVPR2018}} & \multirow{3}{*}{} & \multirow{3}{*}{x} & CNN & 3 & No & No & \multirow{3}{*}{x} & \multirow{3}{*}{} & \multirow{3}{*}{x} \\
 & & & Residual & $2\times10$ & Yes & No & & & \\
 & & & CNN & ($2\times3$) // 2 & No & No & & &  \\ \hline

\cite{TewariCVPR2018} & x & & CNN & 8 & No & No & & & x   \\ \hline
\end{tabularx}
\end{table*}



% \begin{table*}[thp]
% \caption{3D-from-2D face reconstruction approaches based on deep learning - part I.} \label{tab:DL_1}
% % \renewcommand{\arraystretch}{1.3}
% \renewcommand\tabularxcolumn[1]{m{#1}}
% \begin{tabularx}{\textwidth}{XllXXXX}%{Xlp{1.2cm}p{2.45cm}p{2.65cm}p{2.58cm}X}
% \hline
% \multirow{2}{*}{Reference} & \multirow{2}{*}{Year} & \multirow{2}{*}{Images} & \multicolumn{4}{l}{Network}\\ \cline{4-7} 
% & & & Output & Training set & \begin{tabular}[l]{@{}l@{}}Learning\\ framework\end{tabular} & \begin{tabular}[l]{@{}l@{}}Training\\criterion\end{tabular} \\
% \hline
% \citet{SongTIP2012} & 2012 & Single & 3D face & Real 2D-3D & Encoder-decoder & Representations and 3D faces Euclidean loss \\ \hline
% \citet{JourablooCVPR2016} & 2016 & Single & Camera and 3DMM params. & Fit & Cascaded CNN & Parameters Euclidean loss\\ \hline
% \citet{Richardson3DV2016} & 2016 & Single & 3DMM parameters & \textit{Generate\&Render} & Iterative & 3D faces Euclidean loss \\ \hline
% \citet{XZhuCVPR2016} & 2016 & Single & Camera and 3DMM params. & \textit{Fit\&Render} & Cascaded CNN & Weighted parameter distance cost\\ \hline
% \citet{BhagavatulaICCV2017} & 2017 & Single & 3D face and 2D landmarks & \textit{Fit\&Render} & Multi-stage & 3D faces and 2D landmarks Euclidean loss \\ \hline
% \citet{DouCVPR2017} & 2017 & Single & 3DMM parameters & \textit{Generate\&Render} & SubNetworks for specific tasks & 3D faces Euclidean loss\\ \hline
% \citet{GulerCVPR2017} & 2017 & Single & UV-map & \textit{Fit\&Render} & SubNetworks for specific tasks & Residual part L1-loss and quantized part softmax loss\\ \hline
% \citet{JacksonICCV2017} & 2017 & Single & Volumetric representation & \textit{Fit\&Render} & Encoder-decoder & Sigmoid cross entropy \\ \hline
% \citet{JourablooIJCV2017} & 2017 & Single & Camera and 3D params. & Fit & Cascaded CNN & Parameters and 2D landmarks Euclidean loss \\ \hline
% \citet{RichardsonCVPR2017} & 2017 & Single & Camera and 3D params. & \textit{Generate\&Render} & Coarse-to-fine & 3D faces Euclidean loss (coarse) and images Euclidean loss (fine) \\ \hline
% \citet{SelaICCV2017} & 2017 & Single & UV-map (and correspondence with template) & \textit{Generate\&Render} & Feedforward & UV-maps and normals L1-loss \\ \hline
% \citet{TewariICCV2017} & 2017 & Single & Camera, 3DMM and illumination parameters & Unlabelled images & Encoder-decoder & Landmarks and images Euclidean loss \\ \hline
% \citet{TranCVPR2017} & 2017 & Single & 3DMM parameters & Fit multiple images and pool parameters & Feedforward & Asymmetric Euclidean loss \\ \hline
% \citet{TrigeorgisCVPR2017} & 2017 & Single & Surface normals & \textit{Fit\&Render} and \textit{Generate\&Render} & Feedforward & Angular similatiry and \mbox{L1-loss} \\ \hline
% \citet{TranCVPR2018} & 2018 & Single & 3D face & Fit multiple images and pool parameters & Feedforward (coarse) and encoder-decoder (bump) & Asymmetric Euclidean loss (coarse) and bump loss (bump) \\ \hline
% \citet{FLiuCVPR2018} & 2018 & Single & 3D face and identity class & Fit to multiple images forcing equal shape parameters & Encoder-decoder & 3D faces Euclidean loss, softmax loss over identity \\ \hline
% \end{tabularx}
% \end{table*}



% \begin{table*}[thp]
% \caption{3D-from-2D face reconstruction approaches based on deep learning - part II.} \label{tab:DL_2}
% % \renewcommand{\arraystretch}{1.3}
% \renewcommand\tabularxcolumn[1]{m{#1}}
% \begin{tabularx}{\textwidth}{Xlp{1cm}XXXX}
% \hline
% \multirow{2}{*}{Ref.} & \multirow{2}{*}{Year} & \multirow{2}{*}{Images} & \multicolumn{4}{l}{Network}\\ \cline{4-7} 
% & & & Output & Training set & \begin{tabular}[l]{@{}l@{}}Learning\\ framework\end{tabular} & \begin{tabular}[l]{@{}l@{}}Training\\criterion\end{tabular} \\
% \hline
% \citet{KimCVPR2018} & 2018 & Single & Camera, 3DMM and illumination parameters & \textit{Generate\&Render} & Self-supervised bootstrapping & Weighted parameter distance cost\\ \hline
% \citet{LTranCVPR2018} & 2018 & Single & Camera, 3DMM parameters and UV-texture & \textit{Fit\&Render} and unlabelled images & Feedforward and adversarial & Images L1-loss, landmarks euclidean loss \\ \hline
% \citet{SenguptaCVPR2018} & 2018 & Single & Surface normals, albedo and illumination & \textit{Generate\&Render} and unlabelled images & Multi-stage & Images, normals and albedo L1-loss, illumination L2-loss \\ \hline
% \citet{TewariCVPR2018} & 2018 & Single & Camera, 3DMM and illumination parameters & Unlabelled images and landmarks & Feedforward & Images and landmarks euclidean loss \\ \hline
% \citet{YFengECCV2018} & 2018 & Single & UV position map & \textit{Fit\&Render} & Encoder-decoder & UV-maps weighted Euclidean loss \\ \hline
% \citet{YGuoPAMI2018} & 2018 & Single, video & Camera and 3D params. & \textit{Generate\&Render} & Coarse-to-fine & Projected 3D faces Euclidean loss (coarse) and gradients of displacements Euclidean loss (fine) \\ \hline
% \citet{GenovaCVPR2018} & 2018 & Single & 3DMM parameters & \textit{Generate\&Render} and unlabelled images & Encoder-decoder & Weighted parameter distance cost \\ \hline
% \end{tabularx}
% \end{table*}










\section{Other Machine Learning Methods}
% that are not DL and do not use 3DMM (i.e. do not fit a 3DMM)
Although deep learning has been a widely used tool in 3D-from-2D face reconstruction due to its great power, other machine learning methods have been explored.

Some researchers proposed to approach the 3D-from-2D face reconstruction problem as a regression problem, estimating the 3D facial shape from information extracted from the given input image \citep{DouBMVC2014,JeniFG2015,JeniIVC2017,FLiuECCV2016,FLiuFITEE2017,RaraICIP2010,RaraIJCB2011,SanchezCVIM2016,TianFG2018}.

\citep{RaraICIP2010,SanchezCVIM2016,DouBMVC2014} trained regressors using the Partial Least Squares algorithm. \citet{SanchezCVIM2016} proposed to build a regression matrix $\vec{\mathcal{B}}$ that regresses the 3D face surfaces as a linear combination of the contour of the images, $\vec{X} = \vec{C\mathcal{B}}$. The response matrix $\vec{X} \in \mathbb{R}^{M\times3n}$ is built by concatenating the $M$ vectorised 3D training shapes. The predictor matrix $\vec{C} \in \mathbb{R}^{M\times 2l}$ is built by concatenating the pixel locations $(x,y)$ of the 2D contours of the input images (with different poses). After training, this regression matrix can reconstruct a 3D face $\vec{x}$ from the contours of the input images of a subject $\vec{x}$, as $\vec{x}=\vec{\mathcal{B}c}$.

\citet{RaraICIP2010} trained two Partial Least Squares regression models to estimate shape and texture model coefficients from spherical harmonics projection model parameters. The shape and texture models were built applying Principal Component Analysis (PCA) over aligned shapes an textures from the USF 3D Database (similarly to 3D morphable model, see Section \ref{subsubsec:Build3Dmodel}), while the spherical harmonics projection model was built from the input image as explained below. From each image in the same training set $\{\vec{I}_i\}_i$, the reflected light $\vec{B}_i$ is estimated assuming a Lambertian illumination model. Each image can be recovered as a weighted combination of the columns of $\vec{B}_i$, $\vec{I}_i = \vec{B}_i \vec{\upsilon}$. Then, for an input image $\Iin$, solve for $\{\upsilon_i\}_i$ the following equation $\Iin = \vec{B}_i \vec{\upsilon}$ and compute the spherical harmonics projection images $\vec{\mathcal{I}}_i = \vec{B}_i\vec{\upsilon}_i$. From this images, they built a linear model similarly to the shape and texture models.

A similar idea is followed by \citet{DouBMVC2014}. They built two statistical models, one of 2D-landmarks and the other of 3D-landmarks. Thus, their proposed Partial Least Squares regressor estimated coefficients on the 3D-landmarks-model given coefficients on the 2D-landmarks-model. The regressed 3D-landmarks coefficients were then mapped back to $\mathbb{R}^3$ and were used to reconstruct the 3D facial shape by recovering the coefficients of a coupled-dictionary.

Unlike the three previous works, \citet{RaraIJCB2011} used a Principal Component Regression model. However, their proposed approach resembles that of \citep{DouBMVC2014} in the sense that their regressor also estimates coefficients on a 3D shape model from coefficients on a 2D shape model. The main difference is that \citep{RaraIJCB2011} estimates directly parameters on a statistical model built from dense 3D shapes, instead of a model built from sparse sets of 3D landmarks.

\afterpage{\footnotetext[\getrefnumber{first}]{\cite{BhagavatulaICCV2017} compare two different CNNs, one with 8 layers and the other with 16.}}



Contrary to the above approaches that used a single regressor, \citep{JeniFG2015,JeniIVC2017,FLiuECCV2016,FLiuFITEE2017,TianFG2018} proposed a cascade of linear regressors to estimate the 3D shape. \citet{TianFG2018}, similarly to \citep{RaraIJCB2011}, trained a cascade of regressors $\vec{\mathcal{R}}^k$ to predict the shape update $\vec{\Delta}\vec{x}^{k}$ according to the difference between the ground truth 2D landmarks $\vec{\lmk_\text{gt}}$ and the 3D landmarks of the previous shape projected into the image $\vec{\LmkProj}^{,k-1}$, $\vec{x}^{k} = \vec{x}^{k-1} + \vec{\Delta x}^{k} = \vec{x}^{k-1} + \vec{\mathcal{R}}^{k}(\vec{\lmk_\text{gt}} - \vec{\LmkProj}^{,k-1})$. The regressors are trained by minimising the Euclidean distance between the ground truth shape update $\vec{\Delta}\vec{x}^{k}_\text{gt} = \vec{x}_\text{gt} - \vec{x}^{k-1}$ and the estimated shape update by the current regressor over the $M$ training pairs, 
\begin{equation*}
 \vec{\mathcal{R}}^k = \argmin_{\vec{\mathcal{R}}} \sum_{i=1}^M \norm{\vec{\Delta}\vec{x}^{k}_\text{gt} - \vec{\mathcal{R}}(\vec{\lmk_\text{gt}} - \vec{\LmkProj}^{,k-1})}.
\end{equation*}

\citet{JeniFG2015,JeniIVC2017} and \citet{FLiuECCV2016,FLiuFITEE2017} estimated the 2D landmarks in the input image along with the 3D shape. The first \citep{JeniFG2015,JeniIVC2017} used as input a 2D video, reconstructing the 3D face for each frame. They applied a cascaded regressor that estimated a dense set of facial points in the 2D frame, which were in correspondence with the vertices of a 3D face model. Then, the 3D face model was fitted to the frame by minimising the Euclidean distance between the projection of the model vertices and the estimated 2D facial points. \citet{FLiuECCV2016,FLiuFITEE2017} jointly estimated the 2D landmarks and the 3D shape, alternately updating each of them. In each step, the 2D landmarks are updated according to an update estimated by the landmarks regressor $\vec{\mathcal{R}}^k_{\ell}$ from texture features extracted around the landmarks in the input image $h(\Iin,\vec{\ell}^{\text{2D},k-1})$,
\begin{align*}
 \vec{\ell}^{\text{2D},k} &= \vec{\ell}^{\text{2D},k-1} + \vec{\Delta \ell}^{\text{2D},k}\\
 &= \vec{\ell}^{\text{2D},k-1} + \vec{\mathcal{R}}^k_{\ell}(h(\Iin,\vec{\ell}^{\text{2D},k-1})).
\end{align*}
Then, a shape regressor estimates the update of the shape according to the landmarks update, $\vec{x}^k = \vec{x}^{k-1} + \vec{\Delta x}^k = \vec{x}^{k-1} + \vec{\mathcal{R}}^k_{\vec{x}}(\vec{\Delta \ell}^{\text{2D},k})$. Finally, the 2D landmarks were refined by projecting the 3D landmarks on the updated shape assuming a weak perspective projection whose projection matrix is estimated as \begin{equation*}
 \vec{P}^k = \argmin_{\vec{P}} \norm{\vec{\ell}^{\text{2D},k} - \vec{P} \times \vec{\ell}^{\text{3D},k}}.
\end{equation*}

==> Sections/Notation_old.tex <==
% \large

\section*{Notation}
{\doublespacing

\textbf{Model construction}

$M : \#$faces in the model

$N : \#$vertices of the meshes\\\\
\textit{Shape}, $i = 1,\dots,\widetilde{M}$

$\vec{\mathrm{x}}$: shapes in 3D

$\vec{\phi}_i \in \mathbb{R}^{3N}$ : eigenvectors of shape model $\rightarrow \\ \vec{\Phi} =
\begin{pmatrix}
\vdots & & \vdots\\
\vec{\phi}_1 & \cdots & \vec{\phi}_{\widetilde{M}}\\
\vdots & & \vdots
\end{pmatrix} \in \mathbb{R}^{(3N) \times \widetilde{M}}$

$\sigma_{\alpha_i} \in \mathbb{R}$ : eigenvalues of shape model

$\alpha_i \in \mathbb{R}$ : shape model parameters $\rightarrow \vec{\alpha} = (\alpha_1, \dots, \alpha_{\widetilde{M}})$

$\vec{x}(\vec{\alpha})$: 3D face generated by the model shape parameters $\vec{\alpha}$

$\vec{\delta}$: expression model parameters

$\vec{\Upsilon}$: expression model eigenvectors\\\\
\textit{Texture}, $i = 1,\dots,\widetilde{N}$

$\vec{\mathrm{C}}$: textures of the 3D faces (colour)

$\vec{\psi}_i \in \mathbb{R}^{3N}$ : eigenvectors of texture model \\
$\rightarrow \vec{\Psi} \in \mathbb{R}^{(3N) \times \widetilde{N}}$

$\sigma_{\beta_i} \in \mathbb{R}$ : eigenvalues of texture model

$\beta_i \in \mathbb{R}$ : texture model parameters $\rightarrow \vec{\beta} = (\beta_1, \dots, \beta_{\widetilde{N}})$

$\vec{\gamma}_\text{d}$: diffuse lighting parameters

$\vec{\gamma}_\text{s}$: specular lighting parameters\\\\
\textbf{Fitting}

$\Iin$: input image

$\Imod$: rendered image from reconstructed 3D face

$L: \#$landmarks

$\lmk$: landmarks in the input image

$\Lmk$: landmarks in the 3D face

$\LmkProj$: projection of landmarks in the 3D face $\Lmk$ into the image plane 

$\lmkProj$: projection of landmarks in the image $\lmk$ into the 3D face

$\vec{\kappa}$: intrinsic camera parameters (depends on the camera model, but usually focal length, principal point, ...)

$\vec{R}$: rotation matrix

$\vec{\tau}$: translation

$\vec{\zeta} = \{ \vec{R}, \vec{\tau}, \vec{\kappa}\}$: projection parameters (intrinsic and extrinsic)

$\vec{\rho}$: rendering parameters (including $\vec{\kappa}$, $\vec{R}$, $\vec{\tau}$ and illumination parameters)

$\mathcal{P}(\vec{v},\vec{\xi})$: projection of $\vec{v} \in\mathbb{R}^3$ according to parameters $\vec{\xi}$

$\errorI$: distance between $\Iin$ and $\Imod$

$\errorLmk$: distance between $\lmk$ and $\LmkProj$

$\errorReg$: regularisation of the fitting parameters}
